A tensor-train reduced basis solver for parameterized partial differential equations on Cartesian grids

In this manuscript, we introduce the tensor-train reduced basis method, a novel projection-based reduced-order model designed for the efficient solution of parameterized partial differential equations. While reduced-order models are widely used for their computational efficiency compared to full-order models, they often involve significant offline computational costs. Our proposed approach mitigates this limitation by leveraging the tensor train format to efficiently represent high-dimensional finite element quantities. This method offers several advantages, including a reduced number of operations for constructing the reduced subspaces, a cost-effective hyper-reduction strategy for assembling the PDE residual and Jacobian, and a lower dimensionality of the projection subspaces for a given accuracy. We provide a posteriori error estimates to validate the accuracy of the method and evaluate its computational performance on benchmark problems, including the Poisson equation, heat equation, and transient linear elasticity in two- and three-dimensional domains. Although the current framework is restricted to problems defined on Cartesian grids, we anticipate that it can be extended to arbitrary shapes by integrating the tensor-train reduced basis method with unfitted finite element techniques.

==> elasticity_rev.tex <==
\section{Linear Elasticity Equation}
\label{sec: elasticity}

In this section, we briefly discuss the \ac{fom} and \ac{ttrb} implementation in the case of an unsteady, parameterized linear elasticity equation. 
we proceed in a similar fashion as in Sect. \ref{sec: rb} to derive the space-time \ac{fom} for the elasticity problem, which can be expressed as in \eqref{eq: space time FOM}. To define the \ac{ttrb} method, a minor modification is needed to account for the vector-valued nature of the elasticity problem. In fact, a new axis that collects the components of the displacements is necessary to write the snapshots in the ``split-axes'' format. In other words, we consider as snapshot tensor 
\begin{equation}
    \bm{U}_{1,...,d,c,t,\mu} \in \R^{N_1 \times \cdots \times N_d \times N_c \times N_t \times N_{\mu}},
\end{equation} 
where the subscript $c$ stands for ``component'', and $N_c$ denotes the number of components in the vector field ($N_c = d$ in this problem). This implies that the \ac{tt} decomposition for the displacement features an additional 3D core, which serves as a low-rank approximation for the component axis:
\begin{equation}
    \label{eq: elasticity cores}
    \bm{\Phi}_{st,\widehat{t}} = \bm{\Phi}_{\widehat{0},1,\widehat{1}} \cdots \bm{\Phi}_{\widehat{d-1},d,\widehat{d}} \bm{\Phi}_{\widehat{d},c,\widehat{c}} \bm{\Phi}_{\widehat{c},t,\widehat{t}}. 
\end{equation} 
Similarly, the hyper-reduction for the residuals/Jacobians will return the \ac{tt} decompositions
\begin{align}
    \label{eq: elasticity res/jac cores}
    \left\{\bm{\Phi}^{\bm{L}}_{\widehat{0},1,\widehat{1}} \ , \hdots , \bm{\Phi}^{\bm{L}}_{\widehat{d-1},d,\widehat{d}} \ , \bm{\Phi}^{\bm{L}}_{\widehat{d},c,\widehat{c}} \ , \bm{\Phi}^{\bm{L}}_{\widehat{c},t,\widehat{t}}\right\} \ ; \qquad 
    \left\{\bm{\Phi}^{\bm{K}}_{\widehat{0},1,1,\widehat{1}} \ , \hdots , \bm{\Phi}^{\bm{K}}_{\widehat{d-1},d,d,\widehat{d}} \ , \bm{\Phi}^{\bm{K}}_{\widehat{d},c,c,\widehat{c}} \ , \bm{\Phi}^{\bm{K}}_{\widehat{c},t,\widehat{t}}\right\} \ .
\end{align}
As a consequence, the Galerkin projection procedure detailed in Subsection \ref{subs: galerkin projection} increases by one step, due to the presence of the additional component core.
